Generative AI for Programming Education: Benchmarking ChatGPT, GPT-4, and Human Tutors

Generative AI and large language models hold great promise in enhancing computing education by powering next-generation educational technologies for introductory programming. Recent works have studied these models for different scenarios relevant to programming education; however, these works are limited for several reasons, as they typically consider already outdated models or only specific scenario(s). Consequently, there is a lack of a systematic study that benchmarks state-of-the-art models for a comprehensive set of programming education scenarios. In our work, we systematically evaluate two models, ChatGPT (based on GPT-3.5) and GPT-4, and compare their performance with human tutors for a variety of scenarios. We evaluate using five introductory Python programming problems and real-world buggy programs from an online platform, and assess performance using expert-based annotations. Our results show that GPT-4 drastically outperforms ChatGPT (based on GPT-3.5) and comes close to human tutors' performance for several scenarios. These results also highlight settings where GPT-4 still struggles, providing exciting future directions on developing techniques to improve the performance of these models.

==> figs/7_contextualized_explanation/fig_examples_data_new/Q11_p1_ChatGPT.tex <==
In the given program, the specific part you mentioned, `res += y[i]', is responsible for appending the character from string `S2' (`y') to the resultant string `res'. Let's break down the program and provide an explanation of this specific part in the context of the whole program: [...] \textcolor{ExpHighlight}{The while loop iterates until the length of `res' is less than `z'.} [...]


==> figs/7_contextualized_explanation/fig_examples_data_new/Q11_p1_GPT4.tex <==
The specific part `res+=y[i]' is adding a character from the second string `S2' to the merged string `res' [...] \textcolor{ExpHighlight}{The `while' loop runs until the length of the string `res' is less than `z'.} [...]

==> figs/7_contextualized_explanation/fig_examples_data_new/Q11_p1_Tutor.tex <==
The line 'res += y[i]' concatenates to string res the i-th character of string y.

Note that for strings, the += operator is used for concatenation, not addition.

In the larger context of the program, this line is used for alternatively concatenating the characters of strings x and y to the result string, res, initially empty.

More specifically, it handles the concatenation of the characters from y.
